A Survey of Feedback Particle Filter and related Controlled Interacting Particle Systems (CIPS)

In this survey, we describe controlled interacting particle systems (CIPS) to approximate the solution of the optimal filtering and the optimal control problems. Part I of the survey is focussed on the feedback particle filter (FPF) algorithm, its derivation based on optimal transportation theory, and its relationship to the ensemble Kalman filter (EnKF) and the conventional sequential importance sampling-resampling (SIR) particle filters. The central numerical problem of FPF -- to approximate the solution of the Poisson equation -- is described together with the main solution approaches. An analytical and numerical comparison with the SIR particle filter is given to illustrate the advantages of the CIPS approach. Part II of the survey is focussed on adapting these algorithms for the problem of reinforcement learning. The survey includes several remarks that describe extensions as well as open problems in this subject.

==> cut.tex <==

\begin{remark} 
The filter admits a variational structure in the sense that, at each
time $t$, $\phi$ is the unique minimizer of the following variational
problem:
	\begin{equation}\label{eq:Poisson-variational}
		\min_{f \in H^1_0} \mathbb E\left[
                  |\nabla f (\bar X_t)|^2 - f(\bar X_t)(h(\bar X_t) - \mathbb E[h(\bar X_t)])\right]
	\end{equation}
where $H_0^1$ is a suitable Hilbert space (\Sec{sec:gain-approx}).  It is
easy to verify that the Poisson equation is the Euler-Lagrange
equation of the  variational problem.  More directly, the variational
formulation of the gain function is obtained from the optimal
transportion theory (\Sec{sec:OT-FPF-path}).  The
formulation is useful for the purposes of deriving numerical algorithms to
approximate the gain function (\Sec{sec:var-Poisson}). 
%Variational representation is a special characteristic of the Elliptic PDEs such as the Poisson equation.  
\end{remark}



\begin{remark} 
Over the years, we have developed a number of extensions of the basic
FPF algorithm:
\begin{romannum}
\item The formula~\eqref{eq:intro-FPF-Xbar} for the FPF also applies
  to the case where the state $X_t$ lies in a Reimannian manifold,
  such as matrix Lie groups~\citep{zhang2016feedback,zhang2016attitude,zhang2017attitude,zhang2017feedback}.
  In these papers, the FPF is shown to provide an intrinsic
  description of the filter that automatically satisfies the geometric
  constraints of the manifold.  For the special case when the manifold
  is a matrix Lie group, explicit formulae for the filter are derived,
  using the matrix coordinates. Filters for two example problems are
  presented: the attitude estimation problem on $SO(3)$ and the robot
  localization problem in $SE(3)$.
\item The FPF has been  
  extended to handle additional uncertainties in signal and
  measurement model: 
  These extensions, namely, the joint probabilistic data association
  (JPDA)-FPF and the interacting multiple model (IMM) FPF appear
  in~\cite{yang2012joint} and~\cite{yang2013interacting}, respectively.  
\item FPF for finite and discrete state-space appears in~\cite{yang2015feedback}. 
In this setting, the control  input is realized via time-modulated Poisson counter processes. The rate of these Poisson processes are controlled via a feedback control law where the gain solves a linear problem, equivalent to the Poisson equation in the continuous-space. An explicit  characterization of the gain function appears in~\cite{yang2015feedback}.
 
\item The FPF algorithm is also extended for problems that involve $M$ number of non-interacting agents with $M$ number of non-agent specific observations.  In its basic form, the problem is characterized by data association uncertainty whereby the association between the observations and agents must be deduced in addition to the agent state. The FPF algorithm is extended for the large-$M$ limit to derive the equation for the empirical distribution of the hidden agent states. The resulting algorithm is similar to the FPF update-law with additional term that involve the variance of the measurements and a secondary Poisson equation~\citep{kim2020feedback} 

\end{romannum}

\end{remark}

\begin{figure*}[t]
    \centering
%\vspace{-.in}
    \includegraphics[width=1.8\columnwidth]{figures/linear_perf_comp_2}
 %   \vspace{-0.4in}
%\Ebox{.65}{KuraPDEBifurMcD.eps}
%\EBox{.95}{LearningIncoSynR10APhi.eps}
\caption{Comparison of (a) performance and (b) computational time
  between the feedback particle filter (FPF) and the bootstrap particle filter
  (BPF) -- the details of this study appear in~\cite{taoyang_TAC12}.
  In part~(a), the
  performance 
  metric is a normalized mean squared error (mse) in estimating the error covariance.  
  As the number of particles $N$ increases, the mse approaches zero at
  $O(\frac{1}{N})$ for both FPF and the BPF (consistent with the central limit theorem).
  However the performance of FPF is much superior: For the same number
  of particles, there is a 10x improvement in mse.  For the same value
  of mse, the FPF requires 10x fewer particles than that are necessary for
  the BPF.  % The bottom-line is that compared to conventional
  % approaches, FPF gives more accurate results at a lower computational
  % cost. 
%For
%both FPF and BPF, the mse goes to zero as $N\rightarrow\infty$ at
%the rate $\frac{1}{N}$
}
%\vspace{-.4cm}
    \label{f:comp}
\end{figure*}

\begin{remark}
	In its It\^o form, the mean-field
        FPF~\eqref{eq:intro-FPF-Xbar} is expressed as
	\begin{align*}
		\ud \bar{X}_t = &a(\bar{X}_t) \ud t + \ud \bar{B}_t+ \K_t(\bar{X}_t)  (\ud Z_t -
			\frac{h(\bar{X}_t) + \hat{h}_t}{2}\ud t) \\&+ \frac{1}{4}\nabla | \K_t(\Xbar_t)|^2\ud t
	\end{align*}  
where  $\frac{1}{4}\nabla | \K_t(\Xbar_t)|^2$ is the Wong-Zakai
correction term. The It\^o-Stratonovich relationship discussed here is based on interpreting  	$\mathsf K_t(x)$ as a function of space $x$ and time $t$, and interpreting  the
$\circ$ in the Stratonovich form {\em only} with
respect to the space $x$. In a recent paper~\cite[Sec. 3]{pathiraja2020mckean}, the gain
	function is defined and interpreted as a function of space $x$ and
	the density.  This is natural because the dependence upon
	time $t$ comes because of the changes in density ($\bar p_t$) as
	the time evolves.  Because the density is a stochastic process, it is
	argued that the appropriate interpretation of $\circ$ in the
	Stratonovich form should involve {\em both} space $x$ and the density.
	Using such an interpretation, the Stratonovich form invvoles extra-terms that are solutions to accompanying Poisson equations. 
\end{remark}


\begin{remark}
	The finite-$N$ FPF algorithm is an alternative to the sequential
importance resampling (SIR) particle
filters~\citep{gordon93,bain2009,delmoralbook,doucet09}. 
The salient feature of the FPF, compared to the conventional particle
filters, is that the importance sampling and resampling
step is replaced with a feedback control law. Because of this difference,  FPF
does not suffer from the particle degeneracy issue. Also in various
numerical evaluations and comparisons, it has been observed that FPF
exhibits smaller simulation
variance~\citep{berntorp2015,adamtilton_fusion13,yang2013,stano2014}
and better scaling properties with the problem dimension compared to
particle filters~\citep{surace_SIAM_Review,yang2016}.  A comparison
with the BPF, as reported first in our original papers on the subject, appears in \Fig{f:comp}. 
\end{remark}
%\end{remark}
